Posterior Calibrated Training on Sentence Classification Tasks

Most classification models work by first predicting a posterior probability distribution over all classes and then selecting that class with the largest estimated probability. In many settings however, the quality of posterior probability itself (e.g., 65% chance having diabetes), gives more reliable information than the final predicted class alone. When these methods are shown to be poorly calibrated, most fixes to date have relied on posterior calibration, which rescales the predicted probabilities but often has little impact on final classifications. Here we propose an end-to-end training procedure called posterior calibrated (PosCal) training that directly optimizes the objective while minimizing the difference between the predicted and empirical posterior probabilities.We show that PosCal not only helps reduce the calibration error but also improve task performance by penalizing drops in performance of both objectives. Our PosCal achieves about 2.5% of task performance gain and 16.1% of calibration error reduction on GLUE (Wang et al., 2018) compared to the baseline. We achieved the comparable task performance with 13.2% calibration error reduction on xSLUE (Kang and Hovy, 2019), but not outperforming the two-stage calibration baseline. PosCal training can be easily extendable to any types of classification tasks as a form of regularization term. Also, PosCal has the advantage that it incrementally tracks needed statistics for the calibration objective during the training process, making efficient use of large training sets.

==> 00.Abstract.tex <==
\begin{abstract}
%What is the calibration?
%Problem of current neural network
%Problem of current calibration method
%Why NLP didn't care about calibration quality?
Most classification models predict a posterior probability distribution over classes and output the final class with the largest estimated probability.
%by an accuracy of the predicted labels.
%In some practical cases such as self driving cars, however, the quality of posterior probability (e.g., 65\% turn left) itself instead of its categorical decision (e.g., turn left) gives more reliable results for final actions.
In some practical cases such as predicting a diagnosis code, however, the quality of posterior probability (e.g., 65\% chance having diabetes) itself instead of its categorical decision (e.g., has diabetes) gives more reliable results for final actions.
% is crucial because of it reliability.
% Under such evaluation criteria, however, how well the posterior probability estimates capture the true probability is not considered.
%In this case, predicted posterior can be recalibrated by post-processing the outputs.
%\citet{guo2017calibration} showed that the modern neural networks tend to output overconfident posterior as their architectures get complicated.
% For example, appropriately calibrating the posteriors make  \dk{TODO: more motiviational examples}
%Prior methods on posterior calibration are mostly based on rescaling the posterior probability distribution in order to alleviate the miss-calibrated results from the classifier. %, by simply .
Prior methods on posterior calibration are mostly based on rescaling the predicted probability in order to alleviate the miss-calibrated results from the classifier.
The benefits of the classification task are limited because the improved posteriors do not affect the training of the classifier.
%The benefits for the classification task is limited in such two-step post-processing methods because the improved posteriors do not affect the training the classifier.
%Such two-step, post-processing methods are limited not to adapt the potential improvement from the rescaling into the classification task. %\lucas{The wording of this sentence is confusing}
%Here we propose to change the two-stage processes to an end-to-end training procedure called posterior calibrated (\method) training.
Here we propose an end-to-end training procedure called posterior calibrated (\method) training.
% Such methods do not effect on the performance of the classifier. 
%Thus many NLP application that cares only about the performance didn't need to apply such methods.
%What this paper is doing?
% In this paper, we propose a simple but effective optimization method called Posterior Reinforced Training (\method). 
%How PRT Works?
In particular, \method directly optimizes the objective while minimizing the difference between the predicted and empirical posterior probabilities. 
%In particular, \method directly optimizes the objective of the classification task while minimizing the difference between the predicted and empirical posterior probabilities. 
%What did we find?
We show that \method not only helps reduce the calibration error but also improve task performance by penalizing drops in performance of both objectives.  %mutually reinforcing the task-specific and data statistical objectives by combining each other.
Our \method achieves about 2.5$\%$ of task performance gain and 16.1$\%$ of calibration error reduction on GLUE \cite{wang2018glue} compared to the baseline.
We achieved the comparable task performance with 13.2$\%$ calibration error reduction on xSLUE \cite{kang2019xslue}, but not outperforming the two-stage calibration baseline. 
\method training can be easily extendable to any types of classification tasks as a form of regularization term.
Also, \method has the advantage that it incrementally tracks needed statistics for the calibration objective during the training process, making efficient use of large training sets. 
% on the training objective (e.g., a regularization).
% Our proposed method also can be easily extended to any types of classifiers which output the posterior probability, as an additional term of the training loss like a regularizer.
%\taehee{Last comment!}
% \dk{This abstract is great! But, it needs to be shorten a little bit?}
The code is publicly available\footnote{\url{https://github.com/THEEJUNG/PosCal/}}.
\end{abstract}

%\hua{test}
%\lucas{bbb}
%\thomas{ccc}
